Canonical Paths for MCMC: from Art to Science

Markov Chain Monte Carlo (MCMC) method is a widely used algorithm design scheme with many applications. To make efficient use of this method, the key step is to prove that the Markov chain is rapid mixing. Canonical paths is one of the two main tools to prove rapid mixing. However, there are much fewer success examples comparing to coupling, the other main tool. The main reason is that there is no systematic approach or general recipe to design canonical paths. Building up on a previous exploration by McQuillan, we develop a general theory to design canonical paths for MCMC: We reduce the task of designing canonical paths to solving a set of linear equations, which can be automatically done even by a machine. Making use of this general approach, we obtain fully polynomial-time randomized approximation schemes (FPRAS) for counting the number of $b$-matching with $b\leq 7$ and $b$-edge-cover with $b\leq 2$. They are natural generalizations of matchings and edge covers for graphs. No polynomial time approximation was previously known for these problems.

==> markovchain.tex <==
\section{Markov Chain and Canonical Path}
\label{sec:markov}

In the section, we briefly describe the markov chain used in
\cite{mcquillan2013approximating} and its construction of canonical
paths.

Let $\Lambda=(G(V,E),(f_v)_{v\in V})$ be an instance with $\abs{V}=n$
and every $f_v$ is windable. Let $\mathcal{E}$ be the set of half
edges in $G$. The state space of the chain is
$\Omega=\Omega_0\cup \Omega_2$. For every two configuration
$\sigma,\pi\in\Omega$, the transition probability $P(\sigma,\pi)$ is
defined as
\[
  P(\sigma,\pi)=
  \begin{cases}
    \frac{2}{n^2}\min\tuple{1,\frac{w_\Lambda(\pi)}{w_\Lambda(\sigma)}}
    &\mbox{if }d(\sigma,\pi)=2\\
    1-\frac{2}{n^2}\sum_{\rho:d(\sigma,\rho)=2}\min\tuple{1,\frac{w_\Lambda(\rho)}{w_\Lambda(\sigma)}} & \mbox{if }\sigma=\pi\\
    0 & \mbox{otherwise,}
  \end{cases}
\]
where $d(\sigma,\pi)$ denote the Hamming distance between $\sigma$ and
$\pi$.

For every $\sigma\in\Omega$, we denote
$\mu_\Lambda(\sigma)\defeq\frac{w_\Lambda(\sigma)}{Z_0+Z_2}$ and for
every set $S\subseteq \Omega$, we denote
$\mu_\Lambda(S)\defeq\sum_{\sigma\in S}\mu_{\Lambda}(\sigma)$.

The following rapid mixing result for above chain was established in
\cite{mcquillan2013approximating}.

\begin{theorem}
  For all $\sigma\in\Omega$ and all non-negative integers $t$, we have
  \[
    \sum_{\pi\in\Omega}\abs{P^t(\sigma,\pi)-\mu_\Lambda(\pi)} \le
    \tuple{\mu_\Lambda(\sigma)}^{-\frac{1}{2}}\exp{-t\cdot\mu_\Lambda(\Omega_0)^2/n^4}.
  \]
\end{theorem}

The result was proved by a canonical path argument, we sketch the
construction of canonical paths here.

\bigskip
\noindent\textbf{Flow from $\Omega_0$ to $\Omega$.} Let
$\sigma\in\Omega_0$ and $\pi\in\Omega_2$ be two configurations and
$z=\sigma\oplus\pi$. Consider a tuple
$\tuple{M_v\in \mathcal{M}_{z\cap\mathcal{E}(v)}}_{v\in V}$, define
$T$ as the set of singletons in $\bigcup_{v\in V}M_v$, i.e.,
$T\defeq\set{S\in M_v\mid v\in V\mbox{ and }S\mbox{ is a singleton}}$.
We fix a partition of $T$ into pairs (note that $|T|$ is even by the definition of $\Omega_0$ and $\Omega_2$) and denote the partition as
$M'$.  Define $M\defeq\bigcup_{v\in V}M_v\cup M'\in\mathcal{M}_z$, we
call $M$ the partition induced by
$\tuple{M_v\in \mathcal{M}_{z\cap\mathcal{E}(v)}}_{v\in V}$.

Then for every tuple
$\tuple{M_v\in \mathcal{M}_{z\cap\mathcal{E}(v)}}_{v\in V}$, we define
a canonical path $\gamma_{\sigma,\pi,M}$ where $M\in\mathcal{M}_z$ is
the partition induced by the tuple as follows: We first construct a
graph $G_{M,z}=(V_z,E_M)$ where

\begin{itemize}
\item $V_z=\set{e_v\in \mathcal{E}\mid z(e_v)=1}$;
\item $E_M=M\cup \set{\set{e_u,e_v}\in V_z^2\mid \set{u,v}\in E}$.
\end{itemize}
Since both $\sigma,\pi\in\Omega$, which implies $G_{M,z}$ is a graph
consisting of disjoint cycles and a path.  We recursively choose an
order of edges $\set{e_1,e_2,\dots,e_m}$ in $E_M$ as follows:
\begin{itemize}
\item If there is a unique path $P=(e_1,e_2,\dots,e_k)$, then start
  from $e_1$ and choose edges along the path in the same order. After
  this is done, remove $P$.
\item If there is no path, choose a cycle $C=(e_1,e_2,\dots,e_k,e_1)$
  such that $\set{e_1,e_2}\in M$. Then start from $e_1$ and choose
  edges along the cycle. After this is done, remove $C$.
\end{itemize}
This order induce an order of pairs in $M$. We
denote it by $\set{S_1,S_2,\dots, S_t}$ where each $S_k\in M$ is a
pair of half edges.

For every $k=0,1,2,\dots,t$, let $E_k\defeq \bigcup_{i=1}^kS_k$.  We
then construct a flow-path $\gamma_{\sigma,\pi,M}$ in $\Omega$ as
\[
  \sigma=\sigma\oplus E_0\to \sigma\oplus E_1\to\dots\to\sigma\oplus
  E_t=\pi,
\]
and equip the path with weight
\[
  \wt{\gamma_{\sigma,\pi,M}}=\prod_{v\in
    V}B_v(\sigma|_{\mathcal{E}(v)},\pi|_{\mathcal{E}(v)},M_v)/(Z_0+Z_2)^2,
\]
where for every $v\in V$, $B_v(\cdot,\cdot,\cdot)$ is the set of
values witnessing $f_v$ is windable.

Then for every $\sigma\in \Omega_0$ and $\pi\in\Omega$, it holds that
\begin{align*}
  \sum_{M\in\mathcal{M}_z}\wt{\gamma_{\sigma,\pi,M}}
  &=\frac{1}{(Z_0+Z_2)^2}\cdot \sum_{\set{M_v\in \mathcal{M}_{z\cap \mathcal{E}(v)}}_{v\in V}}\prod_{v\in V}B_v(\sigma|_{\mathcal{E}(v)},\pi|_{\mathcal{E}_v},M_v)\\
  &=\frac{1}{(Z_0+Z_2)^2}\cdot\prod_{v\in V}\sum_{M_v\in\mathcal{M}_{z\cap\mathcal{E}(v)}}B_v(\sigma|_{\mathcal{E}(v)},\pi|_{\mathcal{E}(v)},M_v)\\
  &\overset{(\heartsuit)}{=}\frac{1}{(Z_0+Z_2)^2}\cdot\prod_{v\in V}f_v(\sigma|_{\mathcal{E}(v)})f_v(\pi|_{\mathcal{E}(v)})\\
  &=\mu_\Lambda(\sigma)\mu_{\Lambda}(\pi),
\end{align*}
where $(\heartsuit)$ is due to the definition of windability.

% First consider the function $F$ defined on $\mathcal{E}$ where for
% every $\sigma\in\set{0,1}^{\mathcal{E}}$:
% \[
%   F(\sigma)=
%   \begin{cases}
%     \prod_{v\in V}f_v\tuple{\sigma|_{\mathcal{E}(v)}} & \mbox{if $\|\sigma\|$ is even.}\\
%     0 & \mbox{otherwise.}
%   \end{cases}
% \]





% % The following lemma was proved in
% % \cite{mcquillan2013approximating}.

% % \begin{lemma}\label{lem:global-even-windable}
% %   If the instance $\Lambda$ satisfies the conditions specified in
% %   Theorem \ref{thm:rapidmixing}, then for every
% %   $\sigma,\pi\in\set{0,1}^{\mathcal{E}}$ and every
% %   $M\in\mathcal{M}_{\sigma\oplus \pi}$, there exist values
% %   $B(\sigma,\pi,M)$ such that
% %   \begin{enumerate}
% %   \item $F(\sigma)F(\pi)=\sum_{M\in\mathcal{M}_{\sigma\oplus
% %     \pi}}B(\sigma,\pi,M)$ for all
% %     $\sigma,\pi\in\set{0,1}^{\mathcal{E}}$, and
% %   \item $B(\sigma,\pi,M)=B(\sigma\oplus S,\pi\oplus S,M)$ for all
% %     $\sigma,\pi\in\set{0,1}^{\mathcal{E}}$ and all $S\in
% %     M\in\mathcal{M}_{\sigma\oplus \pi}$.
% %   \end{enumerate}
% % \end{lemma}

% \noindent \textbf{Flow from $\Omega_0$ to $\Omega$.} We first
% construct a set of flow from $\Omega_0$ to $\Omega$. Let
% $\sigma\in\Omega_0$, $\pi\in\Omega$ and denote
% $z=\sigma\oplus\pi$. For every $M\in\mathcal{M}_{z}$, we construct a
% graph $G_{M,z}=(V_z,E_M)$ as follows:
% \begin{itemize}
% \item $V_z=\set{e_v\in \mathcal{E}\mid z(e_v)=1}$;
% \item $E_M=M\cup \set{\set{e_u,e_v}\in V_z^2\mid \set{u,v}\in E}$.
% \end{itemize}
% Since both $\sigma,\pi\in\Omega$, which implies $z\in\Omega$ and
% thus $G_{M,z}$ is a graph consisting of disjoint cycles and at most
% one path. We recursively choose an order of edges
% $\set{e_1,e_2,\dots,e_m}$ in $E_M$ as follows:
% \begin{itemize}
% \item If there is an unique path $P=\set{e_1,e_2,\dots,e_k}$, then
%   start from $e_1$ and choose edges along the path in the same
%   order. After this is done, remove $P$.
% \item If there is no path, choose a cycle
%   $C=\set{e_1,e_2,\dots,e_k,e_1}$. Then start from $e_1$ and choose
%   edges along the cycle in one fixed direction . After this is done,
%   remove $C$.
% \end{itemize}

% For every $k=0,1,2,\dots,m$, let
% $E_k\defeq \set{e_1,e_2,\dots,e_k}$.  We then construct a flow-path
% $\gamma_{\sigma,\pi,M}$ in $\Omega$ as
% \[
%   \sigma=\sigma\oplus E_0\to \sigma\oplus E_1\to\dots\to\sigma\oplus
%   E_m=\pi,
% \]
% and equip the path with weight $B(\sigma,\pi,M)/(Z_0+Z_2)^2$, i.e.,
% $\wt{\gamma_{\sigma,\pi,M}}=B(\sigma,\pi,M)/(Z_0+Z_2)^2$. Then it
% follows from Lemma \ref{lem:global-even-windable} that for every
% $\sigma\in\Omega_0$ and $\pi\in\Omega$, the total weight of flow
% from $\sigma$ to $\pi$ is
% \[
%   \sum_{M\in\mathcal{\sigma\oplus\pi}}B(\sigma,\pi,M)/(Z_0+Z_2)^2=F(\sigma)F(\pi)/(Z_0+Z_2)^2=\mu_\Lambda(\sigma)\mu_\Lambda(\pi).
% \]
% We denote $\Gamma_0$ the set of flow-paths constructed above.

\bigskip
\noindent \textbf{Flow from $\Omega$ to $\Omega$.}  For every
$\sigma,\pi\in\Omega$, for every $\rho\in\Omega_0$, every
$M_1\in\mathcal{M}_{\sigma\oplus\rho}$, every
$M_2\in\mathcal{M}_{\rho\oplus\pi}$, we construct a path
$\gamma_{\sigma,\pi,\rho,M_1,M_2}$ which is the concatenation of
$\gamma_{\sigma,\rho,M_1}$ and $\gamma_{\rho,\pi,M_2}$. The weight of
$\gamma_{\sigma,\pi,\rho,M_1,M_2}$ is
$\frac{\wt{\gamma_{\sigma,\rho,M_1}}\wt{\gamma_{\rho,\pi,M_2}}}{\mu_\Lambda(\rho)\mu_\Lambda(\Omega_0)}$. The
flow is legal since
\begin{align*}
  \sum_{\rho\in\Omega_0}\sum_{M_1\in\mathcal{M}_{\sigma\oplus\rho}}\sum_{M_2\in\mathcal{M}_{\rho\oplus\pi}}\wt{\gamma_{\sigma,\pi,\rho,M_1,M_2}}
  &=\sum_{\rho\in\Omega_0}\sum_{M_1\in\mathcal{M}_{\sigma\oplus\rho}}\sum_{M_2\in\mathcal{M}_{\rho\oplus\pi}}\frac{\wt{\gamma_{\sigma,\rho,M_1}}\wt{\gamma_{\rho,\pi,M_2}}}{\mu_\Lambda(\rho)\mu_\Lambda(\Omega_0)}\\
  &=\sum_{\rho\in\Omega_0}\frac{\mu_\Lambda(\sigma)\mu_\Lambda(\rho)\mu_\Lambda(\pi)}{\mu_\Lambda(\Omega_0)}\\
  &=\mu_\Lambda(\sigma)\mu_\Lambda(\pi).
\end{align*}


==> odd.tex <==
\section{Missing Proof Detail for Lemma \ref{lem:2decom}}
  \noindent\textbf{(The case that $m=2n+1$ is odd.)} Let $\mathcal{M}$ denote the
  set of all partitions of $[m]$ into pairs and a singleton. The proof
  for the case that $m$ is odd is similar to the case that $m$ is even, with some
  slight difference on verifying \eqref{eq:sym}, as we have to deal
  with the singleton in each $M\in\mathcal{M}$. We define an
  equivalent relation $\sim$ as that $(x,M)\sim(x',M')$ if
  $k(x,M)=k(x',M')$.
  This definition is the same as the $m=2n$ case as the singleton plays no role.
  For every $k=0,\dots,n$, we also define
  $\Delta_k=\set{(x,M)\mid k(x,M)=k}$
  and claim the the function $H$ is $2$-decomposible if and only if
  for every $0\le k\le n$, there exists $D_k\ge 0$ such that for every
  $x\in\set{0,1}^m$, $H(x)=\sum_{M\in\mathcal{M}}D_{k(x,M)}$. The
  proof for the claim is almost identical as the even case. When verifying
  \eqref{eq:sym}, we can assume no pair $(x_i,x_j)\in M$ with $x_i=x_j=1$
  and that the singleton $(x_i)\in M$ satisfies $x_i=0$ (and the
  same assumption for $(x',M')$), then the remaining argument can go
  through.
%
%  Therefore, the function $H$ is $2$-decomposible if and only if there
%  exist $D_k\ge 0$ for every $k=0,1,\dots,n$ such that for every
%  $x\in\set{0,1}^m$,
%  \[
%    H(x)=\sum_{M\in\mathcal{M}}D_{k(x,M)}=\sum_{k=0}^m\sum_{M\in\mathcal{M}:k(x,M)=k}D_k=\sum_{k=0}^m\abs{\set{M\in\mathcal{M}\mid
%        k(x,M)=k}} D_k.
%  \]
%  Let $i=\sum_{j\in[m]}x_j$, note that
%  \[
%    \abs{\set{M\in\mathcal{M}\mid k(x,M)=k}} =
%    \begin{cases}
%      \binom{i}{j}\binom{2n+1-i}{j}j!(i-j-1)!!(2n+1-i-j)!! & \mbox{if $i\equiv j\pmod 2$;}\\
%      \binom{i}{j}\binom{2n+1-i}{j}j!(i-j)!!(2n-i-j) &
%      \mbox{otherwise},
%    \end{cases}
%  \]
%  this finishes the proof.


\section{Missing Proof Detail for Lemma \ref{lm:nnsol}}
(Case $\mathbf{A}_m\mathbf{x}=(\geq 3)_n\cdot \odd_n$) Let $x_{2j+1}=(1-(-1)^j\frac{(2j+1)!!}{\prod_{i=2}^{j+1}(2n-2i)})\frac{1}{(2n-1)!!}$ ($0\leq j\leq \lfloor\frac{n-1}{2}\rfloor$). Otherwise let $x_{j}=0$. If $j=0$, note that $x_1=0$. If $j=1$, it is not hard to see that $x_3>0$. If $j>1$, we have $n\geq 5$. Observe that the numerator $(2j+1)!!$ is no larger than the denominator $\prod_{i=2}^{j+1}(2n-2i)$ since we have $2j+1\leq 2n-4$. So $x_{2j+1}\geq 0$ always holds. Thus, we prove that $\mathbf{x}$ is a non-negative vector.

The remaining task is to show that $\mathbf{x}$ is exactly the solution. We note
that $x_1=0$ and thus the second equation is satisfied. For $i$ is
  even, it is easy to see that
  $\sum_{0\leq j\leq i}a_{ij} x_{j}=0$ since we have $a_{ij}=0$
  for odd $j$ and $x_j=0$ for even $j$. In the following, we only need to consider the $(2k+1)$th rows ($0\leq k\leq \lfloor\frac{n-1}{2}\rfloor$). In fact, we have the following equalities.
\begin{align*}
&\sum_{0\leq j\leq k}a_{2k+1,2j+1} x_{2j+1}\\
=&\sum_{0\leq j\leq k} a_{2k+1,2j+1}(\frac{1}{(2n-1)!!}+x_{2j+1}-\frac{1}{(2n-1)!!}) \\
\overset{(\heartsuit)}{=}&1+ \sum_{0\leq j\leq k} a_{2k+1,2j+1}(x_{2j+1}-\frac{1}{(2n-1)!!})\\
=& 1+\sum_{0\leq j\leq k} \binom{2k+1}{2j+1} \binom{2n-2k-1}{2j+1} (2j+1)!(2k-2j-1)!! (2n-2k-2j-3)!!(x_{2j+1}-\frac{1}{(2n-1)!!}) \\
=& 1-\sum_{0\leq j\leq k} (-1)^j \frac{(2k+1)!(2n-2k-1)!(n-j-2)!(n-1)}{(k-j)!(n-k-j-1)!j!(2n-1)!} \\
=& 1-\frac{(2k+1)!(2n-2k-1)!(n-1)}{(2n-1)!}\sum_{0\leq j\leq k} (-1)^j \frac{(n-j-2)!}{(k-j)!(n-k-j-1)!j!} \\
\overset{(\diamondsuit)}{=}& 1-\frac{(2k+1)!(2n-2k-1)!(n-1)}{(2n-1)!}\sum_{0\leq j\leq k} \frac{(-1)^j {k \choose j}{n-1-j \choose k}}{n-1-j} = 1-0 = 1.
\end{align*}
where $(\heartsuit)$ is because the sum of entries in each row of $\mathbf{A}_m$ is $(2n-1)!!$ which equals to the total number of partitions, and $(\diamond)$ uses Lemma~\ref{lm:com}.

\section{A Technical Lemma}
\begin{lemma}
\label{lm:com}
$\sum_{j=0}^m \frac{(-1)^j {m \choose j}{n-j \choose m}}{n-j}=0$.
\end{lemma}

\begin{proof}
Consider $f(x)=\sum_{j=0}^m \frac{(-1)^j {m \choose j}{n-j \choose m}x^j }{n-j}$. It is not hard to see that
$$f(x)=\frac{{n\choose m} {}_2F_1(-m,m-n;1-n;x)}{n},$$
where ${}_2F_1(a,b;c;z)=\sum_{i\geq 0}\frac{(a)_i (b)_i}{(c)_i}\cdot \frac{z^i}{i!}$. Here $(a)_i=\prod_{j=0}^{i-1} (a+j)$.

By Equality 15.3.3 in~\cite{abramowitz1965handbook}, ${}_2F_1(-m,m-n;1-n;x)=(1-x)\cdot {}_2F_1(1+m-n,1-m;1-n;x)$. Let $x=1$, we prove the lemma.
\end{proof} 
